Limits on the OH Molecule in the Smith High Velocity Cloud

We have used the Green Bank Telescope (GBT) to search for the OH molecule at several locations in the Smith Cloud, one of the most prominent of the high-velocity clouds that surround the Milky Way. Five positions with a high HI column density were selected as targets for individual pointings, along with a square degree around a molecular cloud detected with the Planck telescope near the tip of the Smith Cloud. Gas in the Galactic disk with similar values of $N_{HI}$ has detectable OH emission. Although we found OH at velocities consistent with the foreground Aquila molecular cloud, nothing was found at the velocity of the Smith Cloud to an rms level of 0.7 mK (T$_b$) in a 1 km $s^1$ channel. The three positions that give the strictest limits on OH are analyzed in detail. Their combined data imply a $5\sigma$ limit on $N(H_2) / N_{HI} \leq 0.03$ scaled by a factor dependent on the OH excitation temperature and background continuum $T_{ex}/(T_{ex}-T_{bg})$. There is no evidence for far-infrared emission from dust within the Smith Cloud. These results are consistent with expectations for a low-metallicity diffuse cloud exposed to the radiation field of the Galactic halo rather than a product of a galactic fountain.

==> OH_obs_table.tex <==

\begin{deluxetable}{cccccc}
	\tablecolumns{6}
	\tablecaption{Observations of the 18cm \oh\ lines  }
\label{tab:OHdata}
\tablehead{\colhead{$\ell$}  & \colhead{$b$} & \colhead{$\sigma T_b (1612)$} &
\colhead{$\sigma T_b (1665)$} & \colhead{$\sigma T_b (1667)$} & \colhead{$\sigma T_b (1721)$} \\
\colhead{($\arcdeg$)} & \colhead{($\arcdeg$)} & \colhead{(mK)} & \colhead{(mK)}  & \colhead{(mK)}  & \colhead{(mK)}    \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)}  & \colhead{(5)} & \colhead{(6)}
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
38.06 & -12.83 & 0.88 & 0.67  & 0.59 & 0.61 \\
%\hline
38.85 & -13.55 & 1.04 & 0.70 & 0.82 & 0.64  \\
%\hline
38.68 & -13.38 & 1.21 & 0.67 & 0.71 & 0.68 \\
%\hline
%38.28 & -12.75 & x & x  \\
%\hline
%38.22 & -12.69 & x & x   \\
xxx &  yyy &  one sq-deg average \\
\noalign{\vspace{5pt}}
\enddata
\tablecomments{Quantities are the rms noise in the spectrum for a 1 \kms\ channel width.
}
\end{deluxetable}


==> OH_obs_table_v2.tex <==
\begin{deluxetable}{cccccc}
	\tablecolumns{6}
	\tablecaption{Observations of the 18cm \oh\ lines  }
\label{tab:OHdata}
\tablehead{\colhead{$\ell$}  & \colhead{$b$} & \colhead{$\sigma T_b (1612)$} &
\colhead{$\sigma T_b (1665)$} & \colhead{$\sigma T_b (1667)$} & \colhead{$\sigma T_b (1721)$} \\
\colhead{($\arcdeg$)} & \colhead{($\arcdeg$)} & \colhead{(mK)} & \colhead{(mK)}  & \colhead{(mK)}  & \colhead{(mK)}    \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)}  & \colhead{(5)} & \colhead{(6)}
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
38.06 & -12.83 & 0.88 & 0.67  & 0.59 & 0.61 \\
%\hline
%\hline
38.68 & -13.38 & 1.21 & 0.67 & 0.71 & 0.68 \\
%\hline
38.85 & -13.55 & 1.04 & 0.70 & 0.82 & 0.64  \\
%\hline

xxx &  yyy &  one sq-deg average \\
\noalign{\vspace{5pt}}
\enddata
\tablecomments{Quantities are the rms noise in the spectrum for a 1 \kms\ channel width.
}
\end{deluxetable}


==> Reddening_table.tex <==
\begin{deluxetable}{ccccccc}
	\tablecolumns{7}
	\tablecaption{Reddening in Directions Searched for OH}
\label{tab:Reddeningdata}
\tablehead{
\colhead{Source} &  \colhead{$\nhi$ (disk)} & \colhead{E(B-V) (IR)\tablenotemark{a}} & 
\colhead{E(B-V) \nhi\ (disk)\tablenotemark{b}} & 
\colhead{Excess E(B-V)\tablenotemark{c}}  & 
\colhead{E(B-V) (Smith)\tablenotemark{d}} & 
\colhead{E(B-V) (Aquilla)\tablenotemark{e}}   \\
\colhead{}  & \colhead{$(10^{20}\cmm)$} & \colhead{(mag)} & 
\colhead{(mag)}  &   \colhead{(mag)} & \colhead{(mag)} & \colhead{(mag)} \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)}  & \colhead{(5)} 
& \colhead{(6)} & \colhead{(7)} \\
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
38.06--12.83 & 8.3 & 0.21 & $0.11\pm .02$ & $0.10 \pm .02$ & $0.06\pm .01$ & $0.5\pm0.1$ \\
38.68--13.38 & 10.2 & 0.20 & $0.14\pm .03$ & $0.06\pm .01$ & $0.08\pm .02$ & $0.12\pm0.03$ \\
38.85--13.55 & 11.2 & 0.25 & $0.15\pm .03$ & $0.10\pm .02$ & $0.06\pm .01$ & $0.14\pm0.03$  \\
%38.28 & -12.75 & $11.6\pm 0.2$ & $13.9\pm 0.4$ & $97.5\pm 0.1$ & 4.7 & 2.0 \\
%38.22 & -12.69 & $13.1\pm 0.1$ & $12.2\pm 0.2$ & $98.4\pm 0.1$ & 4.8 & 2.2 \\ 
\noalign{\vspace{5pt}}
\enddata
\tablenotetext{a}{Reddening from infrared emission \citep{Schlegel1998}.} 
\tablenotetext{b}{Expected reddening from \hi\ only at Galactic disk velocities, omitting the Smith Cloud.} 
\tablenotetext{c}{Reddening in excess of that expected from disk \hi.}
\tablenotetext{d}{Expected reddening from \hi\ in the Smith Cloud assuming its dust is identical to that in the Galactic disk.} 
\tablenotetext{e}{From the low-velocity \oh\ detected from the Aquilla molecular cloud.}
%\tablecomments{ }
\end{deluxetable}


==> Reddening_table_v2.tex <==
\begin{deluxetable}{ccccccc}
	\tablecolumns{7}
	\tablecaption{Reddening E(B-V) in Directions Searched for OH}
\label{tab:Reddeningdata}
\tablehead{
\colhead{Source} &  
%\colhead{$\nhi$ (disk)} & 
\colhead{ \hi\ (disk)\tablenotemark{a}} & 
\colhead{\oh\ (disk)\tablenotemark{b}}  & 
\colhead{Total Foreground} & 
\colhead{ IR\tablenotemark{c}} & 
%\colhead{E(B-V) \nhi\ (disk)\tablenotemark{b}} & 
%\colhead{Excess E(B-V)\tablenotemark{c}}  & 
\colhead{Smith\tablenotemark{d}} &   \\
\colhead{}  & 
\colhead{(mag)} & 
\colhead{(mag)}  &   
\colhead{(mag)} & 
\colhead{(mag)} & 
\colhead{(mag)} \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)}  & \colhead{(5)} 
& \colhead{(6)} \\
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
38.06--12.83  &  $0.11\pm .02$ & $0.20\pm0.01$ & $0.31\pm 0.02$ & 0.18 -- 0.21  & $0.06\pm .01$ \\
38.68--13.38  & $0.14\pm .03$ & $0.09\pm0.01$ & $0.23\pm 0.03$ & 0.17 --  0.20 & $0.08\pm .02$  \\ 
38.85--13.55 & $0.15\pm .03$ & $0.16\pm0.01$ & $0.31\pm 0.03$ & 0.21 -- 0.25 & $0.06\pm .01$  \\
\noalign{\vspace{5pt}}
\enddata
%\tablenotetext{c}{Reddening from infrared emission \citep{Schlegel1998}.} 
\tablenotetext{a}{Expected reddening from \hi\ at Galactic disk velocities, i.e.,  omitting the Smith Cloud.} 
\tablenotetext{b}{From the low-velocity \oh\ detected in the foreground Aquilla molecular cloud.}
\tablenotetext{c}{Reddening from optical and infrared studies averaged over a $5\arcmin$ circle \citep{Schlegel1998,Schlafly2011}.} 
\tablenotetext{d}{Expected reddening from \hi\ in the Smith Cloud assuming its dust is identical to that in the Galactic disk.} 
%\tablecomments{ }
\end{deluxetable}


==> Reddening_table_v3.tex <==
\begin{deluxetable}{|c|ccc|c|c|}
	\tablecolumns{6}
	\tablecaption{Reddening E(B-V) in Directions Searched for OH}
\label{tab:Reddeningdata}
\tablehead{
\colhead{Source} &  
%\colhead{$\nhi$ (disk)} & 
\colhead{ \hi\ (disk)\tablenotemark{a}} & 
\colhead{\oh\ (disk)\tablenotemark{b}}  & 
\colhead{Total Foreground\tablenotemark{c}} & 
\colhead{ IR\tablenotemark{d}} & 
%\colhead{E(B-V) \nhi\ (disk)\tablenotemark{b}} & 
%\colhead{Excess E(B-V)\tablenotemark{c}}  & 
\colhead{Smith\tablenotemark{e}}    \\
\colhead{}  & 
\colhead{(mag)} & 
\colhead{(mag)}  &   
\colhead{(mag)} & 
\colhead{(mag)} & 
\colhead{(mag)} \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)}  & \colhead{(5)} 
& \colhead{(6)} 
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
38.06--12.83  &  $0.11\pm .02$ & $0.020\pm0.003$ & $0.13\pm 0.02$ & 0.18 -- 0.21  & $0.06\pm .01$ \\
38.68--13.38  & $0.14\pm .03$ & $0.008\pm0.002$ & $0.15\pm 0.03$ & 0.17 --  0.20 & $0.08\pm .02$  \\ 
38.85--13.55 & $0.15\pm .03$ & $0.016\pm0.003$ & $0.16\pm 0.03$ & 0.21 -- 0.25 & $0.06\pm .01$  \\
\noalign{\vspace{5pt}}
\enddata
%\tablenotetext{c}{Reddening from infrared emission \citep{Schlegel1998}.} 
\tablenotetext{a}{Expected reddening from foreground \hi, i.e.,  omitting the Smith Cloud.} 
\tablenotetext{b}{Reddening from foreground molecular gas detected in low-velocity \oh\ emission.}
\tablenotetext{c}{Total expected foreground E(B-V), the sum of cols.~2 and 3.}
\tablenotetext{d}{Reddening from optical and infrared studies averaged over a $5\arcmin$ circle \citep{Schlegel1998,Schlafly2011}.} 
\tablenotetext{e}{Expected reddening from \hi\ in the Smith Cloud.} 
%\tablecomments{ }
\end{deluxetable}


==> Reddening_table_v5.tex <==
\begin{deluxetable}{|c|ccc|c|c|}
	\tablecolumns{6}
	\tablecaption{Reddening E(B-V) in Directions Searched for OH}
\label{tab:Reddeningdata}
\tablehead{
\colhead{Position} &  
%\colhead{$\nhi$ (disk)} & 
\colhead{ \hi\ foreground\tablenotemark{a}} & 
\colhead{${\rm H_2}$ foreground\tablenotemark{b}}  & 
\colhead{Total foreground\tablenotemark{c}} & 
\colhead{ IR\tablenotemark{d}} & 
%\colhead{E(B-V) \nhi\ (disk)\tablenotemark{b}} & 
%\colhead{Excess E(B-V)\tablenotemark{c}}  & 
\colhead{Smith\tablenotemark{e}}    \\
\colhead{}  & 
\colhead{(mag)} & 
\colhead{(mag)}  &   
\colhead{(mag) $\Delta T_{ex} = 1$} & 
\colhead{(mag)} & 
\colhead{(mag)} \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)}  & \colhead{(5)} 
& \colhead{(6)} 
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
38.06--12.83  &  $0.109$ & $0.020\Delta T_{ex}$ & $0.13$ & 0.18 -- 0.21  & 0.06 -- 0.07 \\
38.68--13.38  & $0.136$ & $0.008\Delta T_{ex}$ & $0.14$ & 0.17 --  0.20 & 0.08 -- 0.09  \\ 
38.85--13.55 & $0.149$ & $0.016\Delta T_{ex}$ & $0.16$ & 0.21 -- 0.25 & 0.06 -- 0.07  \\
\noalign{\vspace{5pt}}
\enddata
%\tablenotetext{c}{Reddening from infrared emission \citep{Schlegel1998}.} 
\tablenotetext{a}{Expected reddening from foreground \hi, i.e.,  omitting the Smith Cloud.} 
\tablenotetext{b}{Reddening from foreground molecular gas detected in low-velocity \oh\ emission.}
\tablenotetext{c}{Total expected foreground E(B-V), the sum of cols.~2 and 3.}
\tablenotetext{d}{Reddening from optical and infrared studies averaged over a $5\arcmin$ circle \citep{Schlegel1998,Schlafly2011}.} 
\tablenotetext{e}{Expected reddening from \hi\ in the Smith Cloud.} 
%\tablecomments{ }
\end{deluxetable}


==> Reddening_table_v6.tex <==
\begin{deluxetable}{ccc|c|c|c}
	\tablecolumns{6}
	\tablecaption{Reddening E(B-V) in Directions Searched for OH}
\label{tab:Reddeningdata}
\tablehead{
\colhead{Position} &  
%\colhead{$\nhi$ (disk)} & 
\colhead{ \hi\ foreground\tablenotemark{a}} & 
%\colhead{${\rm H_2}$ foreground\tablenotemark{b}}  & 
\colhead{ IR\tablenotemark{b}} & 
\colhead{Difference\tablenotemark{c}} & 
\colhead{${\rm H_2}$ foreground\tablenotemark{d}}  & 
\colhead{Smith\tablenotemark{e}}    \\
\colhead{}  & 
\colhead{(mag)} & 
\colhead{(mag)}  &   
\colhead{(mag)} & 
\colhead{(mag)} & 
\colhead{(mag)} \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)}  & \colhead{(5)} 
& \colhead{(6)} 
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
38.06--12.83  &  $0.11$ &  0.18 -- 0.21 & 0.07 -- 0.10 & $0.020\Delta T_{ex}$  & 0.06 -- 0.07 \\
38.68--13.38  & $0.14$ &  0.17 --  0.20 & 0.03 -- 0.06 & $0.008\Delta T_{ex}$  & 0.08 -- 0.09  \\ 
38.85--13.55 & $0.15$ & 0.21 -- 0.25 & 0.06 -- 0.10 & $0.016\Delta T_{ex}$ & 0.06 -- 0.07  \\
\noalign{\vspace{5pt}}
\enddata
%\tablenotetext{c}{Reddening from infrared emission \citep{Schlegel1998}.} 
\tablenotetext{a}{Expected reddening from foreground \hi, i.e.,  omitting the Smith Cloud.} 
\tablenotetext{b}{Reddening from the infrared emission  \citep{Schlegel1998,Schlafly2011}.} 
\tablenotetext{c}{The difference between cols.~2 and 3.}
\tablenotetext{d}{Reddening from foreground molecular gas detected in low-velocity \oh\ emission.}
\tablenotetext{e}{Expected reddening from the Smith Cloud.} 
%\tablecomments{ }
\end{deluxetable}


==> Smith_LowVel_OH_tab.tex <==
\begin{deluxetable}{ccccccc}
	\tablecolumns{7}
	\tablecaption{Low Velocity OH Detections} 
 \label{tab:OHobservations}
\tablehead{\colhead{Source} & \colhead{Transition} & \colhead{$T_{pk}$} &
\colhead{FWHM} & \colhead{\vlsr} & \colhead{$\rm N_{OH}$}  & \colhead{$\rm \sigma T_b$} \\
\colhead{} & \colhead{(MHz)} & \colhead{(mK)} &   \colhead{($\rm km ~s^{-1}$)} & \colhead{($\rm km ~s^{-1}$)} & 
\colhead{($10^{11}$ \cmm)} & \colhead {(mk)} \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)}  & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} \\
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
38.06-12.83 & 1612  & $-2\pm1$     & $2\pm2$       & $1.8\pm0.6 $  &  --  & 0.88 \\ 
            & 1665  & $12.9\pm0.6$ & $2.5\pm0.1$   & $2.76\pm0.06$ & $154\pm8$ &  0.67 \\
            & 1667 & $27.4\pm0.7$  & $2.33\pm0.07$ & $2.82\pm0.03$ & $186\pm5$ &  0.59  \\ 
            & 1721 & $6.8\pm0.6$   & $2.5\pm0.2$   & $3.7\pm0.1$   &  --  &  0.61 \\
38.68-13.38 & 1612 & $-4\pm11$     & $1\pm4$       & $1.8\pm0.2$   &  --  &  1.04 \\
            &  1665 & $4.3\pm0.7$  & $2.9\pm0.5$   & $1.4\pm0.2$   & $26\pm6$ &  0.70  \\
            &  1667 & $11.6\pm0.7$ & $2.5\pm0.2$   & $1.62\pm0.08$ & $45\pm4$ &  0.82  \\
            &  1721 & $2.5\pm0.5$  & $4\pm1$       & $0.3\pm0.5$   &  --  &  0.64  \\
38.85-13.55 & 1612  & $-3\pm1$     & $3\pm1$       & $0.1\pm0.4$   &  --  &  1.21  \\
            &  1665 & $11.3\pm0.8$ & $2.4\pm0.2$   & $1.36\pm0.08$ & $67\pm6$ &  0.67  \\
            &  1667 & $18.5\pm0.7$ & $2.7\pm0.1$   & $1.16\pm0.05$ & $53\pm3$ &  0.71  \\
            &  1721 & $4.9\pm0.6$ & $2.4\pm0.4$    & $0.6\pm0.2$   &  --  &  0.68  \\
\noalign{\vspace{5pt}}
\enddata
\tablecomments{Quantities $T_{pk}$, FWHM and ${\rm V_{LSR}}$ are from a Gaussian fit to the line. 
$\rm \sigma T_{pk}$ is the rms noise in a 1 \kms\ channel.
$\rm N_{OH}$ is derived from \autoref{eq:NOH} using $\Delta T_{ex} = 1$ and scaled by 9/5 for the 1665 MHz line.
} 
\end{deluxetable}


==> Smith_OH_limits_table.tex <==
\begin{deluxetable}{ccccccc}
	\tablecolumns{7}
	\tablecaption{Limits on \oh\ in the Smith Cloud }
\label{tab:OHabundance}
\tablehead{\colhead{Position} & \colhead{Transition} & \colhead{{\rm $\sigma W(OH)$}} &
\colhead{$\sigma \noh$} & \colhead{$\noh/\nhi$} & 
\colhead{{\rm $N(H_2)$}} & \colhead{{\rm $N(H_2)/\nhi$}} \\
\colhead{($\ell, b$)} & \colhead{(MHz)} & \colhead{(mK-\kms)} &  \colhead{($10^{11} \cmm$)}   & \colhead{$(\rm 5\sigma \ limit)$}
& \colhead{($5\sigma$  limit)} & \colhead{($\rm 5\sigma \ limit$)} \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)}  & \colhead{(5)} & \colhead{(6)} & \colhead{(7)} \\
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
$36\fdg06 -12\fdg83$ & 1665 & 2.6 & 10.6 & $1.1$e-8 & $1.1$e19  & $2.3$e-2 \\ 
                    & 1667 & 2.3 &  5.2 & $5.6$e-9 & $5.2$e18  & $1.1$e-2 \\
$35\fdg85 -13\fdg55$ & 1665 & 2.4 &  9.6 & $1.1$e-8 & $9.6$e18  & $2.1$e-2 \\ 
                    & 1667 & 2.8 &  6.3 & $7.0$e-9 & $6.3$e18  & $1.4$e-2 \\ 
$38\fdg68 -13\fdg38$ & 1665 & 3.0 & 12.2 & $1.0$e-8 & $1.2$e19  & $2.1$e-2 \\ 
                    & 1667 & 2.8 &  6.3 & $5.3$e-9 & $6.3$e18  & $1.1$e-2 \\ 
 \hline\noalign{\vspace{3pt}}
Average            & 1665  & 1.5 &  6.1 & $6.2$e-9 & $6.1$e18 & $1.2$e-2  \\
                   & 1667  & 1.5 &  3.4 & $3.4$e-9 & $3.4$e18 & $6.7$e-3  \\
\hline\noalign{\vspace{3pt}}
Average         & Combined &    &  3.0 &  $3.0$e-9 & $3.0$e18 & $5.9$e-3 \\
\noalign{\vspace{5pt}}
\enddata
\tablecomments{Limits are for $\Delta T_{ex} = 1.0$.  
Average ``combined" limits assume that the 1665 MHz and 1667 MHz transitions are in the LTE ratio.
N$_{\rm H2}$ calculated assuming $\noh /{\rm N_{H2}} = 1.0 \times 10^{-8}$ \citep{Weselak2010,Weselak2022}.
}
\end{deluxetable}


==> Smith_WOH_tab.tex <==
\begin{deluxetable}{lccc}
	\tablecolumns{4}
	\tablecaption{Comparison of 1667 MHz Emission }
 \label{tab:WOH_tab}
\tablehead{\colhead{Source}  & \colhead{$\nhi$} & \colhead{$T_b$} & \colhead{W(1667)} \\ 
\colhead{} & \colhead{($10^{20} \cmm$)} & \colhead{(mK)} &  \colhead{(mK-\kms)}  \\
\colhead{(1)} &  \colhead{(2)} & \colhead{(3)} & \colhead{(4)} \\
}
\startdata
	\hline\hline\noalign{\vspace{5pt}}	
			\noalign{\smallskip}
Smith18 & 3.4 & 40 & 147 \\
B2010 & 4.5 & $\approx 20$ & 136 \\
Smith Cloud & 5.0 & $\leq 2$ & $\leq 6.3$ \\
\noalign{\vspace{5pt}}
\enddata
\tablecomments{ THIS WAS PURSUING A LINE OF THOUGHT THAT IS PROBABLY NOT WORTH FOLLOWING UP.
The Smith18 data are at the position of the brightest \hi\ emission in the cloud studied by \citet{Smith2018}. 
The B2010 data are an average of observations around  $\nhi = 4.5 \times 10^{20} \cmm$ for the Spider cloud from \citet{Barriault2010}.
The limit on $T_b$ and W(OH) for the Smith Cloud is $5\sigma$ for an average of the three pointed positions and a 10  \kms\ line.
} 
\end{deluxetable}

